Weak-to-Strong Generalization Through the Data-Centric Lens

The weak-to-strong generalization phenomenon is the driver for important machine learning applications including highly data-efficient learning and, most recently, performing superalignment. While decades of research have resulted in numerous algorithms that produce strong empirical performance, understanding what aspects of data enable weak-to-strong generalization has been understudied. We propose a simple data-centric mechanism that characterizes weak-to-strong generalization: the overlap density. Intuitively, generalization tracks the number of points that contain overlaps, i.e., both easy patterns (learnable by a weak model) and challenging patterns (only learnable by a stronger model), as with such points, weak predictions can be used to learn challenging patterns by stronger models. We provide a practical overlap detection algorithm to find such points in datasets and leverage them to learn, among multiple sources of data, which to query when seeking to maximize overlap density and thereby enhance weak-to-strong generalization. We present a theoretical result showing that the generalization benefit is a function of the overlap density and a regret bound for our data selection algorithm. Empirically, we validate the mechanism and the overlap detection algorithm on a wide array of settings.

==> old_stuff/overlap_justification_john.tex <==

\paragraph{Justification of Overlap in Synthetic Setting} 

\paragraph{Synthetic Theoretic Details} First, sample $n$ data points $D = \{x_i, y_i\}_i$, from $P(X,Y)$ with equal prior probabilities for $Y = 1$ and $Y = -1$. Then train $f_{weak}$ on $\{P_w x_i, y_i\}_i$, the projection of the dataset onto specifically the weak features. Under this projection, all points from $\cD_{hard}$ are set to 0, while all points from $\cD_{easy}$ and $\cD_{overlap}$ are indistinguishable. Training $f_{weak}$ has the well established result that with probability at least $1-\delta$, 
$$R(f_{weak}) \leq R(f_{weak}^*) + O(\sqrt{\frac{d}{n}\log\frac{n}{d} - \frac{1}{m}\log \delta}),$$
where $d$ is the VC-dimension of the class of $f_{weak}$. The optimal risk of functions in $f_{weak}$ happens to be the Bayes classifier since it can be represented by these weak linear classifiers. This function can be written as
$$
f_{weak}^*(x) = \begin{cases}
    1 & \mu_{easy}^\top x > 0 \\
    -1 & \mu_{easy}^\top x < 0 \\
    -1 & x=0 \text{ or otherwise}
\end{cases}
$$
This third case is an arbitrary choice, since under equal prior probabilities, either choice will have the same risk. Defining $\Phi$ as the normal cdf, we have that 
\begin{align*}
    R(f^*_{weak}) &= (\rho_{easy} + \rho_{overlap})\Phi\left(-\frac{\mu_{easy}^\top \Sigma_{easy} \mu_{easy}}{\mu_{easy}^\top \mu_{easy}}\right) + \frac{\rho_{hard}}{2}
\end{align*}

We now wish to consider the points which the weak model misclassifies, i.e. the detected 'hard points'. These points either are when $Y=1$ and $\mu^\top_{easy}x < 0$, $Y=-1$ and $\mu^\top_{easy}x > 0$, or $Y=-1$ and $\mu^\top_{easy}x = 0$ for hard-only points.



Let $\hat{\mu}$ be the learned weak model parameter and consider the distribution of points from class $Y=1$ marked incorrect by the model, so $\hat{\mu}^\top x < 0$. Our goal is to find the average inner product between this incorrectly labeled points and some correctly labeled point. The distribution of points with the incorrect label of class $Y=1$ follows $X_1 \sim \cD'_{overlap} = \cN(\mu_{overlap}, cI)_{|\hat{\mu}^\top x < 0}$ and $X_2 \sim \cD'_{hard} = \cN(\mu_{hard}, cI_{hard})$. For the expectation of the former distribution, we have

$$
\mathbb{E}[X_1] = \frac{\sqrt{c}}{\Phi(-H)\sqrt{2\pi}} e^{-H^2/2c}
$$

for $H = \frac{\mu^\top \hat{\mu}}{\hat{\mu}^\top \hat{\mu}}$

\paragraph{Synthetic Theoretic Details Try No. 2} We have that, if $U$ and $V$ are independently distributed according to $\cN(\mu^{(U)}, cI)$ and $\cN(\mu^{(V)}, cI)$, 
\begin{align*}
    \mathbb{E}[\|U^\top V\|^2] &= \sum_{i=1}^n \mathbb{E}[(U_i V_i)^2] \\
    &= \sum_{i=1}^n \mathbb{E}[U_i^2]\mathbb{E}[V_i]^2 \\
    &= \sum_{i=1}^n (c + (\mu^{(U)}_i)^2) (c + (\mu^{(U)}_i)^2) \\
    &= \|\mu^{(U)} \odot \mu^{(V)}\|^2 + c\|\mu^{(U)}\|^2 + c\|\mu^{(V)}\|^2 + nc^2
\end{align*}

Don't know if this is helpful yet.

% Also,
% \begin{align*}
%     \text{Var}[U^\top V] &= \sum_{i=1}^n \text{Var}[U_i V_i] \\
%     &= \sum_{i=1}^n c(\mu^{(U)}_i)^2 + c(\mu^{(V)}_i)^2 + c^2 \\
%     &= c\|\mu^{(U)}\|^2 + c\|\mu^{(V)}\|^2 + nc^2
% \end{align*}


%Let $D=\{(x_i, y_i)\}_{i=1}^n$ be a sample from the mixture distribution $P(X,Y)$ as defined above. Let $f_{weak}(x) = \theta_{weak}^\top x$ be some weak classifier parameterized by $\theta_{weak}$ which only has non-zero components in the weak features and classifies $\theta_{weak}^\top x = 0$ as $y=-1$. This is an arbitrary choice as $P(Y=1|\theta_{weak}^\top X = 0) = 0.5$. Let $\cD_{overlap}^{bad, 1}$ be the distribution of $P_{X \sim \cD_{overlap}}(X|Y=1, \theta_{weak}^\top X < 0)$. The expectation of this distribution is
% $$
% \mathbb{E}_{X \sim \cD_{overlap}^{bad, 1}}[X] = \mu - \left(\frac{\sqrt{c}\phi(-p_{\mu})}{\Phi(-p_{\mu})} \right) \frac{\theta_{weak}}{\|\theta_{weak}\|},
% $$
% where $p_{\mu} = \frac{\theta_{weak}^\top \mu}{\|\theta_{weak}\|}$, and $\phi$ and $\Phi$ are the pdf and cdf of $\cN(0, c)$. By the symmetry of the distributions around the origin, $\mathbb{E}_{X \sim \cD_{overlap}^{bad, -1}}[X] = -\mathbb{E}_{X \sim \cD_{overlap}^{bad, 1}}[X]$. We also have for the hard points
% $$
% \mathbb{E}_{X \sim \cD_{hard}^{bad, 1}}[X] = \mu_{hard} - \left(\frac{\sqrt{c}\phi(\|\mu_{hard}\|)}{\Phi(\|\mu_{hard}\|)} \right) \frac{\mu_{hard}}{\|\mu_{hard}\|},
% $$
% and for the easy points,


==> old_stuff/smooth_analysis_John.tex <==

\subsection{Smooth-Data Analysis}
Models inherently understand structure, especially that similar points should have similar labels. 

\begin{defn}[\cite{lang2024theory}] A probability distribution $P$ is said to satisfy $(c,q)$-expansion on sets $(A,B)$ if for any $U \subset B$ with $P(U)>q$, $P(U|B) > cP(\cN(U)|A)$.
\end{defn}

This is the existing result. It's nice, but relies on the concept of data expansion from good points to bad points, which isn't all that intuitive.

\begin{theorem}[\cite{lang2024theory}] Let $\Dg$ be the data points that $f_{weak}$ classifies correctly and $\Db$ be the points $f_{weak}$ classifies incorrectly. Further, let $\cN(\cdot)$ be a neighborhood function. Suppose $P_X$ satisfies $(c,q)$-expansion for $q \leq \frac{3}{4}(1-2\alpha)$ on $(\Dg, \Db)$. Then for any classifier $f$ with $P(f(x) \neq f_{weak}(x) \text{ or } f \text{ not robust at } x) < \frac{1-\alpha+3c\alpha}{4}$, then

$$
R_D(f) \leq \hat{R}_D(f) + \frac{2\alpha}{1-2\alpha}P(\overline{R(f)}|D) + \alpha(1 - \frac{3}{2}c).
$$
\end{theorem}

As long as neighborhoods aren't that large ($s_h$), the data expands.

\begin{lemma}
    Let $\rho'=P(\cN(\Dg)|\Db)$, $\alpha=P(\Db)$, and $s_h=\max_x{P(\cN(x))/P(x)}$. For any $U\subset \Dg$ and $q > 0$, if $P(\Dg \setminus U|\Dg) > q$, then $c=\rho' - \frac{(1-\alpha)(1-q)}{\alpha}s_h$ satisfies
    $$
    P(\cN(\Db \setminus U) | \Dg) > cP(\Db \setminus U | \Db)
    $$
\end{lemma}

\begin{proof}
    \begin{align*}
        P(\cN(\Dg \setminus U) | \Db) &> P(\cN(\Dg)|\Db) - P(\cN(U)|\Db) \\
        &= \rho' - P(\cN(U) \cap \Db) / P(\Db) \\
        &= \rho' - (P(\cN(U) - P(\cN(U) \cap \Dg)) / P(\Db) \\
        &= \rho' - P(\cN(U) / P(\Db) + (P(\cN(U) \cap \Dg)) / P(\Db) \\
        &> \rho' - P(U) s_h / \alpha\\
        &= \rho' - P(U \cap \Dg) s_h / \alpha \\
        &= \rho' - P(U|\Dg)P(\Dg) s_h / \alpha \\
        &> \rho' - (1-q) (1-\alpha) s_h / \alpha \\
        &=c \geq cP(\Dg \setminus U| \Dg) \\
    \end{align*}
\end{proof}

\begin{lemma}
   Let $\rho'=P(\cN(\Dg)|\Db)$, $\alpha=P(\Db)$,  $s_h=\max_x{P(\cN(x))/P(x)}$, $q>0$, and $c=\rho' - \frac{(1-\alpha)(1-q)}{\alpha}s_h$. Then $P$ satisfies $(c,q)$-expansion on $(\Db, \Dg)$.
\end{lemma}

\begin{proof}
    Let $U\subset \Dg$ with $P(U|\Dg)>q$. Define $V = \Dg \setminus U$ so $P(\Dg \setminus V | \Dg) > q$. Then we have 
    $$
    P(\cN(\Db \setminus V) | \Dg) > cP(\Db \setminus V | \Db),
    $$
    and therefore,
    $$
    P(\cN(U) | \Dg) > cP(U | \Db).
    $$
\end{proof}

Replace the requirement for expansion with terms relating to the neighborhood size and reverse overlap density (the neighborhood size of good within bad, rather than the neighborhood size of bad within good).

\begin{theorem}Let $\Dg$ be the data points that $f_{weak}$ classifies correctly and $\Db$ be the points $f_{weak}$ classifies incorrectly. Further, let $\cN(\cdot)$ be a neighborhood function. Then for any classifier $f$ with $P(f(x) \neq f_{weak}(x) \text{ or } f \text{ not robust at } x) < \frac{1-\alpha+3c\alpha}{4}$, then

$$
R_D(f) \leq \hat{R}_D(f) + \frac{2\alpha}{1-2\alpha}P(\overline{R(f)}|D) + \alpha(1 - \frac{3}{2}\rho' + \frac{3(1-\alpha)(1-\frac{3}{4}(1-2\alpha))}{2\alpha}s_h).
$$

This is a stronger bound than the trivial bound $R_D(f) \leq \hat{R}_D(f) + \alpha$ when 

$$
\rho' > \frac{4}{3(1-2\alpha)}P(\overline{R(f)}|D) + \frac{(1-\alpha)(1-q)}{\alpha}s_h.
$$
\end{theorem}

\begin{proof}
     Let $\rho'=P(\cN(\Dg)|\Db)$, $\alpha=P(\Db)$,  and $s_h=\max_x{P(\cN(x))/P(x)}$, and set $q = \frac{3}{4}(1-2\alpha)$ and $c=\rho' - \frac{(1-\alpha)(1-q)}{\alpha}s_h$. Therefore, $P$ satisfies $(c, q)$-expansion on $(\Db, \Dg)$. Since $q \leq \frac{3}{4}(1-2\alpha)$, we can say that 
     $$
    R_D(f) \leq \hat{R}_D(f) + \frac{2\alpha}{1-2\alpha}P(\overline{R(f)}|D) + \alpha(1 - \frac{3}{2}c).
    $$
    We then can substitute in $c$ and obtain the desired result.
\end{proof}

There is an algebraic relationship between the reverse overlap density and the overlap density.

\begin{lemma}
    Let $s_h=\max_x P(\cN(x))/P(x)$. We have
    $$
        P(\cN(\Dg)|\Db) > P(\cN(\Db)|\Dg)(1-\alpha)/(s_h \alpha).
    $$
\end{lemma}

\begin{proof}
    Note that $\cN(\cN(\Dg) \cap \Db) \cap \Dg = \cN(\Db) \cap \Dg$. This is a result of the all points in $\Db$ which have neighbors in $\Dg$ must be mutually neighbored by a point in $\Dg$.

    Therefore
    \begin{align*}
        P(\cN(\Dg)|\Db) &= P(\cN(\Dg)\cap\Db)/P(\Db) \\
        &> P(\cN(\cN(\Dg)\cap\Db))/(s_h P(\Db)) \\
        &> P(\cN(\cN(\Dg)\cap\Db)\cap\Dg)/(s_h P(\Db)) \\
        &= P(\cN(\Db)\cap\Dg)/(s_h P(\Db)) \\
        &= P(\cN(\Db)|\Dg)P(\Dg)/(s_h P(\Db)) \\
        &= P(\cN(\Db)|\Dg)(1-\alpha)/(s_h \alpha). \\
    \end{align*}
\end{proof}

\begin{corollary}
Let $\Dg$ be the data points that $f_{weak}$ classifies correctly and $\Db$ be the points $f_{weak}$ classifies incorrectly. Further, let $\cN(\cdot)$ be a neighborhood function and $\rho=P(\cN(\Db)|\Dg)$. Then for any classifier $f$ with $P(f(x) \neq f_{weak}(x) \text{ or } f \text{ not robust at } x) < \frac{1-\alpha+3c\alpha}{4}$, then

$$
% R_D(f) \leq \hat{R}_D(f) + \frac{2\alpha}{1-2\alpha}P(\overline{R(f)}|D) + \alpha(1 - \frac{3(1-\alpha)}{2\alpha}(\frac{\rho}{s_h}+(1-\frac{3}{4}(1-2\alpha))s_h)).
R_D(f) \leq \hat{R}_D(f) + \frac{2\alpha}{1-2\alpha}P(\overline{R(f)}|D) + \alpha - \frac{3(1-\alpha)\rho}{2s_h} + \frac{3(1-\alpha)(1-\frac{3}{4}(1-2\alpha))}{2}s_h.
% R_D(f) \leq \hat{R}_D(f) + \frac{2\alpha}{1-2\alpha}P(\overline{R(f)}|D) + \alpha(1 - \frac{3(1-\alpha)\rho}{2\alpha s_h} + \frac{3(1-\alpha)(1-\frac{3}{4}(1-2\alpha))}{2\alpha}s_h).
$$

\end{corollary}

\subsection{Analysis on overlap identification}

TODO. For the original detection algorithm and feature importance method, I have this. It's nothing fancy. All it says is if you learn a linear model, the top features should be detectable with not much worse than standard Hoeffding-like decay. This is unchecked, so please comment or remove before submission in unfixed and unchecked.

\begin{align*}
    P(\text{top-k violated}) &\leq P(\bigcup_{i\in [k], j\in [n-k]} \hat{w}_i < \hat{w}_j) \\
    &\leq \sum_{i\in [k]} \sum_{j\in [n-k]} P(\hat{w}_i < \hat{w}_j | w^*_j > w^*_j) \\ 
    &\leq \sum_{i\in [k]} \sum_{j\in [n-k]} 2e^{-nr_{ij}^2} \\ 
    &\leq 2k(n-k)e^{-n\min_{i\in [k], j\in [n-k]}(r_{ij})^2} \\ 
    &= 2k(n-k)e^{-nr_{k,k+1}^2} \\ 
\end{align*}


==> old_stuff/theorem42backup.tex <==

\begin{theorem}
Assume that we are sampling points from each of these distributions all of the same class. Given the above setup, $\E[\Xov^T \Xho ]-\E[\Xeo^T \Xho]=\norm{\tilde{\mu}_{hard}}_{2}^2$. Furthermore, it holds that
\begin{itemize}
    \item For small deviations $(0 \leq t \leq \frac{2\nu^2}{b})$, \[P\left(\Xov^T \Xho-\Xeo^T \Xho)\leq \norm{\tilde{\mu}_{hard}}_{2}^2-t \right) \leq 2^{d/2}\exp{\left(-\frac{t^2}{2\nu^2}\right)}\]
    \item For large deviations $(t > \frac{2\nu^2}{b})$,\[P\left(\Xov^T \Xho-\Xeo^T \Xho)\leq \norm{\tilde{\mu}_{hard}}_{2}^2-t \right) \leq 2^{d/2}\exp{\left(-\frac{t}{2b}\right)},\] 
\end{itemize}
where $b = 2c$ and $\nu = \sqrt{c}(1+\sqrt{2})\|\muh\|$.
\end{theorem}

% \begin{theorem}
% Assume that we are sampling points from each of these distributions all of the same class. Given the above setup, $\E[\Xov^T \Xho ]-\E[\Xeo^T \Xho]=\norm{\tilde{\mu}_{hard}}_{2}^2$. Furthermore, it holds that
%  \[P\left(\Xov^T \Xho-\Xeo^T \Xho)\leq \norm{\tilde{\mu}_{hard}}_{2}^2-t \right) \leq \exp{\left(-\min(\frac{t^2}{2\nu^2}, \frac{t}{2b})+\frac{d}{2}\log 2\right)}\]
%     % \item For large deviations $(t > \frac{2\nu^2}{b})$,\[P\left(\Xov^T \Xho-\Xeo^T \Xho)\leq \norm{\tilde{\mu}_{hard}}_{2}^2-t \right) \leq 2^{d/2}\exp{\left(-\frac{t}{2b}\right)},\] 
% , where $b = 2c$ and $\nu = \sqrt{c}(1+\sqrt{2})\|\muh\|$.
% \end{theorem}

% Original theorem
% \begin{theorem}
% Assume that we are sampling points from each of these distributions all of the same class. Given the above setup, $\E[\Xov^T \Xho ]-\E[\Xeo^T \Xho]=\norm{\tilde{\mu}_{hard}}_{2}^2$. Furthermore, it holds that
% \begin{itemize}
%     \item For small deviations $(0 \leq t \leq \frac{\nu^2}{b})$, \[P\left(\Xov^T \Xho-\Xeo^T \Xho)\leq \norm{\tilde{\mu}_{hard}}_{2}^2-t \right) \leq \sqrt{2}\exp{\left(-\frac{t^2}{2\nu^2}\right)}\]
%     \item For large deviations $(t > \frac{\nu^2}{b})$,\[P\left(\Xov^T \Xho-\Xeo^T \Xho)\leq \norm{\tilde{\mu}_{hard}}_{2}^2-t \right) \leq \sqrt{2}\exp{\left(-\frac{t}{2b}\right)},\] 
% \end{itemize}
% where $\nu=d_{hard}+2c\norm{\tilde{\mu}_{hard}}^2_2$, $b=c+2\sqrt{c}\norm{\tilde{\mu}_{hard}}_{\infty}$
% \end{theorem}

\begin{proof}
Let $\Xdiff = \Xov - \Xeo$ so that
$$
\E[\Xov^T \Xho ]-\E[\Xeo^T \Xho] = \E[\Xdiff^\top \Xho]
$$
This difference distribution will follow $\Xdiff \sim \cN(\mu_{\text{overlap}} - \mu_{\text{easy only}}, 2cI) = \cN(\muh, 2cI)$. 

% Consequently, we have

% \begin{align*}
%     \E[\Xdiff^\top \Xho] &= \|\muh\|^2 \\
%     \text{Var}[\Xdiff^\top \Xho] &= \sum_{i=1}^{d_{\text{easy}} + d_{\text{hard}}} \text{Var}[(\Xdiff)_i (\Xho)_i] \\
%     \text{Var}[\Xdiff^\top \Xho] &= \sum_{i=1}^{d_{\text{easy}} + d_{\text{hard}}} \text{Var}[(\Xdiff)_i] \E[\Xho]^2 + \text{Var}[(\Xho)_i] \E[\Xdiff]^2 + \text{Var}[(\Xdiff)_i] \text{Var}[(\Xho)_i] \\
%     &= \sum_{i=1}^{d_{\text{easy}} + d_{\text{hard}}} 4c (\muh)_i^2 + c (\muh)_i^2 + 4c^2 \\
%     &= 5c \|\muh\|^2 + 4(d_{\text{easy}} + d_{\text{hard}})c^2. \\
% \end{align*}

Consider one of the independent coordinates $i$ and let $X_1 \sim \cN(\mu_1, \sigma^2_1)$ and $X_2 \sim \cN(\mu_2, \sigma^2_2)$, where $\mu_1 = (\mu_{\text{diff}})_i = (\mu_{\text{hard only}})_i$, $\sigma^2_1 = \text{Var}[(\Xdiff)_i] = 2c$, $\mu_2 = (\mu_{\text{hard only}})_i$, and $\sigma^2_2 = \text{Var}[(\Xho)_i] = c$. 
Let $\xi_1$ and $\xi_2$ be standard normally distributed so the above distributions follow
\begin{align*}
    X_1 &= \mu_1 + \sigma_1 \xi_1 \\
    X_2 &= \mu_2 + \sigma_2 \xi_2. \\
\end{align*}

Therefore, $X_1X_2 - \E[X_1X_2] = \mu_2\sigma_1\xi_1 +\mu_1\sigma_2\xi_2 + \sigma_1\sigma_2\xi_1\xi_2$. We now investigate the moment generating function (MGF) of $X_1X_2 - \E[X_1X_2]$. 

\begin{align*}
    \E[e^{\lambda(X_1X_2 - \E[X_1X_2])}] &= \E[e^{\lambda(\mu_2\sigma_1\xi_1 +\mu_1\sigma_2\xi_2 + \sigma_1\sigma_2\xi_1\xi_2)}] \\
    &= \E_{\xi_1}[e^{\lambda (\mu_2\sigma_1\xi_1)} \E_{\xi_2}[e^{\lambda (\mu_1\sigma_2\xi_2 + \sigma_1\sigma_2\xi_1\xi_2)} | \xi_1]] \\
    &= \E_{\xi_1}[e^{\lambda (\mu_2\sigma_1\xi_1)} \E_{\xi_2}[e^{\lambda (\mu_1 + \sigma_1\xi_1)\sigma_2\xi_2} | \xi_1]] \\
    &= \E_{\xi_1}[e^{\lambda (\mu_2\sigma_1\xi_1)} e^{(\lambda (\mu_1 + \sigma_1\xi_1)\sigma_2)^2/2}] \\
    &= \E_{\xi_1}[e^{\lambda^2 \mu_1^2 \sigma_2^2/2} e^{(\lambda \mu_2 \sigma_1 + \lambda^2 \sigma_1 \sigma_2^2 \mu_1)\xi_1} e^{(\lambda^2\sigma_1^2\sigma_2^2/2)\xi_1^2}]. \\
\end{align*}

For notational simplicity, let $A=\lambda^2\sigma_1^2\sigma_2^2/2$, $B=\lambda \mu_2 \sigma_1 + \lambda^2 \sigma_1 \sigma_2^2 \mu_1$, and $C=\lambda^2 \mu_1^2 \sigma_2^2/2$. We then have (TODO, what?? Probably needs a citation),
$$
\E[e^{C + B\xi_1 + A\xi_2^2}] = \frac{1}{\sqrt{1-2A}}e^C e^{\frac{B^2}{2(1-2A)}}, \quad \text{for }2A < 1,
$$
which is useful for deriving the sub-exponential coefficients of $X_1X_2$. From $\lambda^2\sigma_1^2\sigma_2^2 = 2A < 1$, we have that $|\lambda| < \frac{1}{\sigma_1 \sigma_2}$. Substituting in $A$, $B$, and $C$, 
\begin{align*}
    \E[e^{\lambda(X_1X_2 - \E[X_1X_2])}] &= \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{\lambda^2 \mu_1^2 \sigma_2^2/2 + \frac{(\lambda \mu_2 \sigma_1 + \lambda^2 \sigma_1 \sigma_2^2 \mu_1)^2}{2(1 - \lambda^2\sigma_1^2\sigma_2^2)}} \\
    &= \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2 \mu_1^2 \sigma_2^2 - \lambda^4\sigma_1^2\sigma_2^4 \mu_1^2 + (\lambda \mu_2 \sigma_1 + \lambda^2 \sigma_1 \sigma_2^2 \mu_1)^2}{2(1 - \lambda^2\sigma_1^2\sigma_2^2)}} \\
    &= \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2 \mu_1^2 \sigma_2^2 - \lambda^4\sigma_1^2\sigma_2^4 \mu_1^2 + \lambda^2 \mu_2^2 \sigma_1^2 + 2\lambda^3 \mu_1 \mu_2 \sigma_1^2 \sigma_2^2 + \lambda^4 \sigma_1^2 \sigma_2^4 \mu_1^2}{2(1 - \lambda^2\sigma_1^2\sigma_2^2)}} \\
    &= \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2 \mu_1^2 \sigma_2^2 + \lambda^2 \mu_2^2 \sigma_1^2 + 2\lambda^3 \mu_1 \mu_2 \sigma_1^2 \sigma_2^2}{2(1 - \lambda^2\sigma_1^2\sigma_2^2)}} \\
    &= \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2 \mu_1^2 \sigma_2^2 + \lambda^2 \mu_2^2 \sigma_1^2 + 2\lambda^3 \mu_1 \mu_2 \sigma_1^2 \sigma_2^2}{2(1 - \lambda^2\sigma_1^2\sigma_2^2)}} \\
    &= \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2}{2}(\frac{\mu_1^2 \sigma_2^2 + \mu_2^2 \sigma_1^2 + 2\lambda \mu_1 \mu_2 \sigma_1^2 \sigma_2^2}{1 - \lambda^2\sigma_1^2\sigma_2^2})} \\
    &\leq \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2}{2}(\frac{\mu_1^2 \sigma_2^2 + \mu_2^2 \sigma_1^2 + 2\mu_1 \mu_2 \sigma_1 \sigma_2}{1 - \lambda^2\sigma_1^2\sigma_2^2})} \\
    &= \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2}{2}(\frac{(\mu_1\sigma_2 + \mu_2\sigma_1)^2}{1 - \lambda^2\sigma_1^2\sigma_2^2})} \\
\end{align*}

To further simplify this bound, assume that $|\lambda| \leq \frac{1}{\sqrt{2}\sigma_1\sigma_2}$ so $\frac{1}{1 - \lambda^2 \sigma_1^2 \sigma_2^2} \leq 2$. Therefore

\begin{align*}
    \E[e^{\lambda(X_1X_2 - \E[X_1X_2])}] &\leq \frac{1}{\sqrt{1 - \lambda^2\sigma_1^2\sigma_2^2}}e^{ \frac{\lambda^2}{2}(\frac{(\mu_1\sigma_2 + \mu_2\sigma_1)^2}{1 - \lambda^2\sigma_1^2\sigma_2^2})} \\
    &\leq \sqrt{2} e^{ \frac{\lambda^2}{2}(2(\mu_1\sigma_2 + \mu_2\sigma_1)^2)} \\
    &\leq \sqrt{2} e^{\lambda^2(\mu_1\sigma_2 + \mu_2\sigma_1)^2} \\
\end{align*}

Substituting in the original coordinates of $\Xdiff$ and $\Xho$, we have

\begin{align*}
    \E[e^{\lambda((\Xdiff)_i(\Xho)_i - (\muh)_i^2)}] &\leq \sqrt{2} e^{\lambda^2(\sqrt{c}(\muh)_i + \sqrt{2c}(\muh)_i)^2} \\
    & \leq \sqrt{2} e^{\lambda^2c(1 + \sqrt{2})^2(\muh)_i^2}. \\
\end{align*}

Thus, for independent coordinates with identical variances, we have

\begin{align*}
    \E[e^{\lambda(\Xdiff^\top \Xho - \|\muh\|^2)}] &\leq 2^{d/2} e^{\lambda^2c(1 + \sqrt{2})^2\|\muh\|^2}, \\
\end{align*}
when $|\lambda| \leq \frac{1}{\sqrt{2}(\sqrt{2c})(\sqrt{c})} = \frac{1}{2c}$. Let $b = 2c$ and $\nu = \sqrt{c}(1+\sqrt{2})\|\muh\|$.

By Chernoff's inequality, we have that
\begin{align*}
    P(\Xdiff^\top \Xho - \|\muh\|^2 \geq t) &\leq e^{-\lambda t} \E[e^{\lambda(\Xdiff^\top \Xho - \|\muh\|^2}] \\
    &\leq 2^{d/2} e^{-\lambda t + \lambda^2c(1 + \sqrt{2})^2\|\muh\|^2}, \\
\end{align*}
for every $\lambda \in [0, \frac{1}{2c}]$. The optimal value of $\lambda$ when unconstrained is $\lambda^* = \frac{t}{2c(1 + \sqrt{2})^2\|\muh\|^2}$. First, if $\lambda^* \leq \frac{1}{2c}$, then we have
\begin{align*}
    P(\Xdiff^\top \Xho - \|\muh\|^2 \geq t) &\leq 2^{d/2} e^{-\lambda^* t + (\lambda^*)^2c(1 + \sqrt{2})^2\|\muh\|^2} \\
    &\leq 2^{d/2} e^{-\frac{t^2}{2c(1 + \sqrt{2})^2\|\muh\|^2} + \frac{t^2}{4c(1 + \sqrt{2})^2\|\muh\|^2}}\\
    &= 2^{d/2} e^{-\frac{t^2}{4c(1 + \sqrt{2})^2\|\muh\|^2}}\\
    &= 2^{d/2} e^{-\frac{t^2}{(2\nu)^2}},
\end{align*}
and $\lambda^* \leq \frac{1}{2c} \Rightarrow t \leq (1 + \sqrt{2})^2\|\muh\|^2 = \frac{2\nu^2}{b}$.

Otherwise, the constrained minimum will be found at the upper bound of $\lambda = \frac{1}{2c}$. Therefore,
\begin{align*}
    P(\Xdiff^\top \Xho - \|\muh\|^2 \geq t) &\leq 2^{d/2} e^{-\lambda t + \lambda^2c(1 + \sqrt{2})^2\|\muh\|^2} \\
    &\leq 2^{d/2} e^{-\frac{t}{2c} + \frac{c}{4c^2}(1 + \sqrt{2})^2\|\muh\|^2} \\
    &\leq 2^{d/2} e^{-\frac{t}{4c}} \\ 
    &= 2^{d/2} e^{-\frac{t}{2b}}, 
\end{align*}
where the penultimate inequality comes from $\lambda^* > \frac{1}{2c} \Rightarrow t > (1 + \sqrt{2})^2\|\muh\|^2 = \frac{2\nu^2}{b}$. We therefore arrive at the desired bound.

% Reference original proof:

% Define $\Xdiff=\Xov-\Xeo$. Then $\Xdiff$ follows the same distribution as $\Xho$. Consequently, we have\[\E[\Xdiff^T\Xho]=\norm{\tilde{\mu}_{hard}}_{2}^2,\]
% \[Var[\Xdiff^T\Xho]=d_{hard}c^2+2c\norm{\tilde{\mu}_{hard}}_{2}^2\]
% Furthermore, the product of two Gaussian random variables follows a subexponential distribution.Specifically, $\Xov^T \Xho \sim SE(\nu^2, b)$, where $\nu=d_{hard}+2c\norm{\tilde{\mu}_{hard}}^2_2$, $b=c+2\sqrt{c}\norm{\tilde{\mu}_{hard}}_{\infty}$. Therefore, the result follows Bernstein's inequality \citep{vershynin2018high}.

\end{proof}


==> old_stuff/theory_eta_robust_backup.tex <==

\paragraph{Notations.}
 $\rvx$ refers to a random variable with distribution $\cD$ and italicized letters $\vx$ refer to realizations of $\rvx$.
We will assume for ease of exposition that the input space $\cX$ is a discrete\footnote{This is done to simplify some of the arguments, as in \citet{haochen2021provable}. As shown there, the results can be generalized to continuous $\cX$ with additional regularity conditions.
Our bounds have no dependence on $|\cX|$.} (but possibly very large) set, such as all vectors in $\mathbb{R}^d$ up to a fixed numerical precision.
For $A\subset \cX$ we use $\widebar{A} = \cX \setminus A$.
We assume there is a ground-truth function of interest, $y: \cX \to \cY = \{1,\ldots,k\}$, and a \textit{pseudolabeler} $\hy: \cX \to \cY$, which assigns to each point $\vx$ a label. We assume that there is no abstention. 
Let $\{S_i\}$ be a partition of $\cX$ such that within each $S_i$, the ground-truth label is constant.
For example, we could set $S_i = \{\vx | y(\vx) = i \}$ to be the set of points with ground-truth label $i$.
Each $S_i$ can be further partitioned into the correctly-pseudolabeled examples $S_i^{good} = \{\vx \in S_i | \tilde{y}(\vx) = y(\vx)\}$ and the incorrectly-pseudolabeled examples $S_i^{bad} = S_i \setminus S_i^{good}$. 
For two classifiers $f, g: \cX \to \cY$ and a set $U \subset \cX$, we use 
$\err(f,g | U)$ to represent $\P(f(\rvx) \ne g(\rvx) | \rvx \in U)$,
their probability of disagreement in the set $U$.

\begin{definition}[$\eta$-robust]\label{def:eta-robust}
For an arbitrary classifier $f$ and point $\vx$, define $r(f,\vx) = \P(f(\rvx') \ne f(\vx) | \rvx' \in \cN(\vx))$ as the probability $f$ gives different labels to $\vx$ and a random neighbor $\rvx'$ of $\vx$.
    A classifier $f: \cX \to \cY$ is said to be $\eta$-robust at a point $\vx$ if $r(f,\vx) \le \eta$.
    For an arbitrary classifier $f$, let $R_{\eta}(f) = \{\vx : r(f,\vx) \le \eta\}$ be the set of $\eta$-robust points for $f$.
\end{definition}
\begin{definition}[$\eta$-robust neighborhood size]
Let $A, U \subset \cX$. The size of the $\eta$-robust neighborhood of $U$ in $A$ is:
$
    P_{1-\eta}(U,A) := \min_{V\subset \cX}\{\P(V|A) : w(V,U) \ge (1-\eta)w(\cN(U),U)\}.
$
\end{definition}

\begin{definition}[Expansion]
\label{def:relative-expansion}
Fix sets $A,B \subset \cX$. 
We say the distribution $\P_\rvx$ satisfies $(c,q)$-expansion on $(A,B)$ if for all sets $U \subset B$ with $\P(U|B) > q$,
$\P(\cN(U) | A) > c\P(U|B)$.
\end{definition}


\begin{definition}[Expansion of a set collection]
\label{def:relative-expansion-family}
Fix sets $A, B \subset \cX$ and suppose $\cM$ is a collection of subsets of $B$. 
Then we say $\cM$ satisfies $(c,q)$-expansion on $(A,B)$ if all sets $U\in \cM$ with $\P(U|B)>q$ satisfy $\P(\cN(U) | A) > c\P(U|B)$.
\end{definition}
\begin{definition}[Robust expansion]
Fix sets $A, B \subset \cX$ and suppose $\cM$ is a collection of subsets of $B$. $\cM$ satisfies $(c,q,\eta)$-robust expansion on $(A,B)$ if for all $U \in \cM$ with $\P(U|B) >q$, $P_{1-\eta}(U,A) > c\P(U|B)$. This exactly recovers Definition \ref{def:relative-expansion-family} when $\eta=0$.
\end{definition}

\begin{definition}[Expanding set family]
Let $\cF$ be the hypothesis class for the strong model, $y$ the ground-truth function, and $B\subset \cX$ an arbitrary set.
For each $f\in \cF$ let $U(B,f) = \{\vx \in B : f(\vx) \ne y(\vx)\}$ be the set of $f$'s mistakes on $y$ in $B$.
Then we define the family:
\[
\cM_{\eta}(B, \cF) = \{R_{\eta}(f) \cap U(B,f) : f \in \cF\}.
\]
Similarly, we define:
\[
\cM_{\eta}'(B, \cF) = \{R_\eta(f) \cap (B \setminus U(B,f)) : f \in \cF\}
\]
as the family of $\eta$-robust non-mistake sets.
\end{definition}


\paragraph{Problem Setup.}
Suppose the input space can be partitioned into easy, hard, and overlap density, i.e. $\cX = \De \cup \Dh \cup \Do$. We assume that the pseudolabeler's accuracy is the same in the easy and overlapping regions ($\De$ and $\Do$), and is higher in these regions compared to the hard region ($\Dh$). Specifically, we have:
\[\varepsilon_1 = P(y(\rvx)\neq \hy(\rvx)|S_i \cap \De)=P(y(\rvx)\neq\hy(\rvx)|S_i \cap \Do) \leq  P(y(\rvx)\neq\hy(\rvx)|S_i \cap \Dh)=\varepsilon_2\]
We assume that $ 0 < \varepsilon_1 \leq \varepsilon_2 \leq 0.5 $.
Further, denote the proportion of partitions as
\[\pe=P(\De|S_i)\]
\[\ph=P(\Dh|S_i)\]
\[\po=P(\Do|S_i)\]

Our goal is to show how the overlap density can make strong model perform better in $p^{hard}_i$ based on (robust) expansion property. Our main assumption is $\cM'_\eta(S_i^{good} \cap \Do, \cF)$ satisfies $(c, q, \eta)$ robust expansion on $(\Sb \cap \Dh, \Sg \cap \D_{overlap})$. It captures our intuition that strong model can learn something useful for hard data points from overlap data points.

In this setup, the trivial error bound obtained by perfectly mimicking the weak pseudolabeler is \[\err(f, y|S_i)= (\pe + \po)\varepsilon_1 + \ph \varepsilon_2 .\] Our claim is that $\err(f, y|S_i \cap \Dh) < \varepsilon_2$ when the expansion coefficient $c$ --- which represents generalization from overlap density to hard density --- is large, and the model error rate in overlap density is low, leading to better performance of the weak-to-strong model. Now we state our main theorem.


\begin{theorem}\label{thm:pseudolabel_correction} Suppose $\cM'_\eta(S_i^{good} \cap \Do, \cF)$ satisfies $(c,q,\eta)$-robust expansion on $(\Sb\cap \Dh, \Sg\cap \Do)$ for some $c > 0$ and $\eta \geq 0$. Consider an arbitrary classifier $f$ such that $\P(f(\rvx)\neq \hy(\rvx)$ or $f$ not $\eta$-robust at $\rvx$|$S_i \cap \Do) \leq 1-q-\varepsilon_1$. then $f$ satisfies the following error bound:
\begin{align*}
\err(f, y|S_i \cap \Dh) &\leq \err(f, \hy|S_i \cap \Dh) + \varepsilon_2 \\
&-2c\varepsilon_2 \left(1- \err(f, \hy|S_i^{good} \cap \Do)- \P(\overline{R_\eta(f)}|S_i^{good} \cap \Do)\right)
\end{align*}
% \begin{align*}
% \err(f, y|S_i \cap \Dh) &\leq \err(f, \hy|S_i \cap \Dh) + \varepsilon_2 \\
% &+2c\varepsilon_2 \left(\err(f, y|S_i^{good} \cap \Do)+ \P(\overline{R_\eta(f)}|S_i^{good} \cap \Do) - 1\right)
% \end{align*}
% \begin{align*}
% \err(f, y|S_i \cap \Dh) &\leq \err(f, \hy|S_i \cap \Dh) + (1-2c)\varepsilon_2 \\
% &+2c\varepsilon_2 \err(f, y|S_i^{good} \cap \Do)+2c\varepsilon_2 \P(\overline{R_\eta(f)}|S_i^{good} \cap \Do)
% \end{align*}
\end{theorem}

The proof is in Appendix \ref{app:theory}.

Note that the trivial bound on $\err(f, y|S_i \cap \Dh)$ is $\err(f, y|S_i \cap \Dh) \leq \err(f, \hy|S_i \cap \Dh) + \varepsilon_2$. Theorem \ref{thm:pseudolabel_correction} implies weak-to-strong generalization is facilitated as long as the overlap density expands well (large $c$), the the error rate in correct overlap density is low (small $\err(f, y|S_i^{good} \cap \Do)$, and $f$ is more robust in correct overlap density (small $\P(\overline{R_\eta(f)}|S_i^{good} \cap \Do)$). \todo{We include an empirical justification of expansion property in a synthetic setup, in Appendix \ref{app:exp_details}.}

